LLMs as Meta-Reviewers' Assistants: A Case Study

One of the most important yet onerous tasks in the academic peer-reviewing process is composing meta-reviews, which involves assimilating diverse opinions from multiple expert peers, formulating one's self-judgment as a senior expert, and then summarizing all these perspectives into a concise holistic overview to make an overall recommendation. This process is time-consuming and can be compromised by human factors like fatigue, inconsistency, missing tiny details, etc. Given the latest major developments in Large Language Models (LLMs), it is very compelling to rigorously study whether LLMs can help metareviewers perform this important task better. In this paper, we perform a case study with three popular LLMs, i.e., GPT-3.5, LLaMA2, and PaLM2, to assist meta-reviewers in better comprehending multiple experts perspectives by generating a controlled multi-perspective summary (MPS) of their opinions. To achieve this, we prompt three LLMs with different types/levels of prompts based on the recently proposed TELeR taxonomy. Finally, we perform a detailed qualitative study of the MPSs generated by the LLMs and report our findings.

==> Sections/Background.tex <==
\section{Background on TELeR Taxonomy}\label{sec:background}


As shown in Figure~\ref{TELeR_Fig}, the taxonomy introduced by \citet{santu2023teler} categorizes complex task prompts based on the following four criteria. 

\begin{enumerate}[leftmargin=*,itemsep=0.2ex,partopsep=0.2ex,parsep=0ex]
    
    \item \textbf{Turn}: This refers to the number of turns or shots used while prompting an LLM to accomplish a complex task. In general, prompts can be classified as either single or multi-turn.
    
    \item \textbf{Expression}: This refers to the style of expression for interacting with the LLM, such as questioning or instructing. 
    
    \item \textbf{Level of Details}: This dimension of prompt style deals with the granularity or depth of question or instruction. Prompts with higher levels of detail provide more granular instructions. For example, Level 0 has no directive, i.e., questions or instructions. On the other hand, Level 4 prompts have to specify the particular sub-tasks, few-shot examples, and/or the basis for evaluating the output generated by the LLM.
    
    \item \textbf{Role}: Some LLMs provide users with the option of specifying the system's role. The response of LLM can vary due to changes in role definitions although the prompt content remains unchanged.
\end{enumerate}

%For more details on the TELeR taxonomy and its applications, see \cite{santu2023teler}.



==> Sections/Case.tex <==
\begin{figure*}[!htb]\scriptsize
    \centering
    
    \begin{tcolorbox}[enhanced jigsaw,unbreakable,pad at break*=1mm,
colback=blue!5!white,colframe=blue!75!black,title=Review No. 1]\scriptsize
    
    \underline{\textbf{Summary of the paper}}: The authors propose to improve the sample quality of autoregressive models. The authors propose to (1) - smooth the input data distribution leveraging methods that have shown success in adversarial defense, (2) recover input distribution by learning to reverse the smoothing process. The authors first demonstrate the efficiency of their method on 1d toy-problem, and extend the demonstration to more complex datasets such as MNIST, CIFAR-10 and CelebA with application such as image generation, inpaintting and denoising.

    \smallskip
    
    \underline{\textbf{Pros}}: The idea to leverage a method previously used for adversarial defense to density estimation is interesting and novel. The paper is well motivated through the manifold hypothesis approximation (which results in densities with high Lipschitz constants) and compounding errors. The theory is strong.
    
    \smallskip
    
    \underline{\textbf{Cons}}: The experiments on denoising and inpainting are only qualitative and suffer from a lack of quantitative evaluation.

    \smallskip
    \underline{\textbf{Recommendation}:} The article is clear, well motivated, and have a strong theoretical grounding. Therefore I would tend to accept the article.
    
    \smallskip
    \underline{\textbf{Detailed comments}}: The experiment on 2d synthetic datasets (especially the olympic dataset) should be discussed more thoroughly. First, it is not clear that the proposed model is generating better sample than the MADE baseline on this specific dataset. Second, the intersection between rings, in the olympic dataset, seems to be much poorly modeled with the proposed approach compared to the MADE baseline. What is the reason ?
    
    In the section 3.2 the authors are introducing 2 different debiasing methods (either a denoising step or another autoregressive model). In the rest of the article it is not clear which of the two methods the authors are using. In addition, in the 2d toy-problem (i.e. ring and olympic) as the authors are choosing a gaussian smoothing both debiasing methods are usable. Therefore it would be interesting to show both methods and to describe thoroughly the differences (in addition, it might provide an answer to my previous point ...
    
    \end{tcolorbox}
    \caption{Review Number 1 (Review Date: 10/24/2020) \santu{move these to appendix}\sanjeev{moved to appendix}}  
    \smallskip
    \smallskip
    \label{tab:my_label}
    \centering
    \smallskip
    \smallskip
    
\begin{tcolorbox}[enhanced jigsaw, unbreakable, pad at break*=1mm, colback=blue!5!white, colframe=blue!75!black, top=0mm, title=Review No. 2]\scriptsize
\underline{\textbf{Summary}}: Autoregressive models have demonstrate their potential utility for modeling images and other types of complex data with high flexibility (particularly in density estimation). However, its sampling ability is not that good as explained in the paper. Authors show that one of the main weaknesses of autoregressive models comes from the propagation of mistakes due to the mismatch of conditionals. Inspired in the promising results of randomized smoothing in adversarial models (Cohen et al. 2019), authors propose a similar strategy. The addition of Gaussian noise and posterior modeling of the smoother data makes easier to the autoregressive density to capture the true data distribution. The benefits of this strategy are empirically proved and shown in the experiments.

\underline{\textbf{Strengths}}: The quality of writing is high and the presentation of the paper facilitates the process of reading. I have to say that I enjoyed while reviewing it. The analysis and description of problems for sampling from autoregressive models is completely understandable to me and I agree with the manifold hypothesis held. Results with the “sharp” multimodal data looks reliable to me and I believe that the smoother process can also reduce the lipschitz constant as stated in Theorem 1. Until pp. 5, nothing is said about the data denoising process, so one could initially think that there is no way to recover the target density without noise, but authors also did an effort on this. Good point. It is important to remark that the randomized smoothing process can be reverted once learning finishes. Additionally, I particularly like how authors first present the idea on 1-d examples, later in the experiments, the method is validated with 2-d rings and finally, as stated in the introduction, with different image datasets. Finally, I did not find any similar work that mixes the idea of smoothing for improving autoregressive modelling.

\smallskip
\underline{\textbf{Weaknesses, Questions \& Recommendations}}: To me, there are 3 main points of weakness: [W1]. A lack of analysis about the optimal noise for randomized smoothing. [W2]. Why just Gaussian noise, what if data is discrete, could we do this with another type of noise? [W3]. Comments about denoising are included a bit late in the manuscript. I think that authors should remark that this is a reversible process.

\smallskip
\underline{\textbf{My main questions are}}: [Q1]. In section 2.2, I do not see why data closer to the manifold should have larger first order derivatives or even infinity. Is this a bit counter intuitive, or not? Like, better positioned, worse gradient values? [Q2]. Is the 1/N term in the global likelihood expression of 1st paragraph of section 2 correct? [Q3]. If I do not appropriately choose the $\sigma$ parameter for smoothing, do I have the risk of not capturing some modes of the original data? I have the opinion that adding too much or too less noise to data could “mask” modes and something could be lost. Am I correct? Did authors empirically analyzed this in the experiments? [Q4]. How could we assess that conditionals are now better fitted than before?

\smallskip
\underline{\textbf{A few recommendations for improvement}}: [Rec1]. I would explain a bit more the manifold hypothesis of section 2.2, maybe a diagram or figure would help for quicker comprehension of the problem. [Rec2]. Some acronym for “randomized smoothing” would help in the 1st paragraph of section 3.1. To avoid repetitive expressions.
\end{tcolorbox}
\caption{Review Number 2 (Review Date: 10/25/2020) \santu{move these to appendix}\sanjeev{moved to appendix}}
\label{fig:my_label}

\end{figure*}





\begin{figure*}[!htb] \scriptsize

\begin{tcolorbox}[enhanced jigsaw,unbreakable,pad at break*=1mm,
colback=blue!5!white,colframe=blue!75!black,title=Review No. 3,
  ]
\smallskip
\underline{\textbf{SHORT DESCRIPTION}};
This paper proposes a two-stage generative modeling approach, first learning a distribution over noised data, then learning the original data distribution conditioned on this noised data. The paper demonstrates that this leads to improved sample quality compared to fitting the data distribution directly.

\smallskip
\underline{\textbf{DISCUSSION}}: Overall, I like this paper: it's a straightforward idea, decently motivated and fairly well described, and has good supporting empirical evaluation. I didn't expect the sampling performance to improve substantially by adding just a single denoising step, and I think demonstrating this is a good contribution. However, I think the paper could be improved by some more careful discussion, and a better placement in the literature.

"Theorem 2 shows that our smoothing process provides a regularization effect on the original objective... This regularization effect can, intuitively, increase the generalization capability of the model." How does the extra term in the theorem lead to a regularization effect? Why does this 'intuitively' increase the generalization capability of the model? Unless I'm mistaken, the added term is (up to a constant) the Laplacian of the log-likelihood w.r.t. data. The objective maximizes this on average across observed data, which intuitively minimizes the 'curvature' or 'steepness' of the log-likelihood at observed data, thus presumably smoothing the maximum likelihood solution. This Laplacian term also appears in the score matching objective presented in Theorem 1 of 'Estimation of Non-Normalized Statistical Models by Score Matching, Hyvarinen 2005', where it is minimized instead of maximized. There are also known connections between score matching and denoising methods e.g. 'Optimal Approximation of Signal Priors, Hyvarinen 2006', and 'A Connection Between Score Matching and Denoising Autoencoders, Vincent 2011', which you've cited in passing later. Much of this material and how it relates to the objective in Theorem 2 might be discussed in more depth rather than passing over it as simply a 'regularization term'.

"Our approach is related to two-stage VAE (Dai \& Wipf, 2019) which introduces a second VAE to correct the errors made by the first VAE." I'm not sure I agree with this. The idea of the two-stage VAE in that paper is to clean up mismatch between the aggregate posterior q(z) and the prior p(z). On the other hand, your variational model is identical to the canonical VAE setup: x is data, z is noised data, the 'posterior' q(z | x) is fixed and adds Gaussian noise, the 'prior' p(z) is a powerful autoregressive model, and the observation likelihood p(x | z) is another powerful autoregressive model (the canonical VAE would have learned q(z | x), fixed simple p(z), and learned but simple p(x | z)). This is one of the reasons 'VAE' can a confusing term when used to describe latent variable generative models in general: assuming something should be 'encoded' and 'decoded' can sometimes obfuscate the actual probabilistic model. What you propose in this paper might generically be called a 'denoising VAE', but again that's maybe not the most accurate description. I think the most closely related work is probably the denoising diffusion and denoising score-matching approaches which have received attention recently and which you've mentioned, but you could also think of it as turning a denoising autoencoder into a generative model. In any case, I think a more careful discussion of these points would be beneficial for the paper.

Finally, the approach isn't really tied to autoregressive models, apart from the motivation given in terms of smoothing 1D distributions. It's fairly likely that the same idea could readily be applied to e.g. normalizing flows and that it would work well there also, so it would have been nice to see experiments featuring flows included here. This would be especially useful since your best-performing two-stage method takes autoregressive models, which are already slow samplers, and effectively doubles their sampling time.

\underline{\textbf{EXTRA NOTES}}: Maybe be careful ...
\end{tcolorbox}

\caption{Review Number 3 (Review Date: 10/27/2020) \santu{move these to appendix}\sanjeev{moved to appendix}}
    \label{fig:my_label2}
\end{figure*}

